What makes math problems hard for reinforcement learning: a case study

Using a long-standing conjecture from combinatorial group theory, we explore, from multiple perspectives, the challenges of finding rare instances carrying disproportionately high rewards. Based on lessons learned in the context defined by the Andrews-Curtis conjecture, we propose algorithmic enhancements and a topological hardness measure with implications for a broad class of search problems. As part of our study, we also address several open mathematical questions. Notably, we demonstrate the length reducibility of all but two presentations in the Akbulut-Kirby series (1981), and resolve various potential counterexamples in the Miller-Schupp series (1991), including three infinite subfamilies.

==> app/counterexamples.tex <==
% !TEX root = ../ac_paper.tex

\section{Potential Counterexamples}

While we focused on a subset of presentations from the Miller-Schupp series in this paper, there are a 

We mentioned some potential counterexamples of the Andrews-Curtis conjecture in the main text in section 2.2. Here, we mention some other potential counterexamples. 

A third series of potential counterexamples is due to Gordon \cite{Brown}:
\[
\G(m, n, p, q) \colon \angles{x, y \mid x = [x^m, y^n],\ y = [y^p, x^q]}.
\]
where $m,n,p,q \in \mathbb{Z}$.
All examples of this series with the total relator length of 14 are known
to be AC-trivializable \cite{Bowman-McCaul}
\footnote{Perform the same exercise as in the footnote above for this series.}
\newline






==> app/profiles.tex <==
% !TEX root = ../ac_paper.tex

\section{Persistent homology profiles}\anibal{@self: Add the new examples when available}

It is natural to base the AC-graph at a potential counterexample to the AC conjecture.
Let \(\Sigma^\ell\) be the full subgraph of \(\Gamma^{\text{AC(2)}}\) containing all presentation that can be joined to \(AK(3)\) through a path whose maximum length is at most \(\ell\).
In \cref{fig:ak_classic_persistence} and \cref{fig:ak_prime_persistence} we respectively present the number of vertices, edges, and isolated components of \(\Sigma^\ell\) constructed using classic and prime moves.

\begin{figure}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$\ell$ & $v(\ell)$ & $e(\ell)$ & $ic(\ell,1)$ & $ic(\ell,2)$ & $ic(\ell,3)$ & $ic(\ell,4)$ & $ic(\ell,5)$ & $ic(\ell,6)$ \\ \hline
		15 & 6864 & 20762 & 1 &  &  &  &  &  \\ \hline
		16 & 10280 & 31090 & 4 & 1 &  &  &  &  \\ \hline
		17 & 428904 & 1297682 & 68 & 27 & 2 & 4 &  &  \\ \hline
		18 & 1007496 & 3047669 & 122 & 27 & 10 & 4 &  &  \\ \hline
		19 & 11804992 & 35738752 & 498 & 115 & 30 & 16 & 12 & 1 \\ \hline
		20 & 25705728 & 77795370 & 826 & 147 & 46 & 28 & 32 & 1 \\ \hline
	\end{tabular}
	\caption{Isolated components with respect to base \(\AK(3)\) in the AC graph constructed with classic moves.}
	\label{fig:ak_classic_persistence}
\end{figure}

\begin{figure}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$\ell$ & $v(\ell)$ & $e(\ell)$ & $ic(\ell,1)$ & $ic(\ell,2)$ & $ic(\ell,3)$ & $ic(\ell,4)$ & $ic(\ell,5)$ & $ic(\ell,6)$ \\ \hline
		15 & 1716 & 3474 & 1 &  &  &  &  &  \\ \hline
		16 & 10280 & 20824 & 16 & 4 & 3 &  &  &  \\ \hline
		17 & 428904 & 870176 & 232 & 82 & 17 & 4 &  &  \\ \hline
		18 & 1007496 & 2043912 & 360 & 94 & 37 & 4 &  &  \\ \hline
		19 & 11804992 & 23962672 & 1664 & 364 & 106 & 16 & 24 & 1 \\ \hline
		20 & 25705728 & 52149632 & 2760 & 476 & 170 & 40 & 56 & 1 \\ \hline
		21 & 109521488 & 222218112 & 5016 & 1804 & 378 & 72 & 56 & 17 \\ \hline
	\end{tabular}
	\caption{Isolated components with respect to the base \(\AK(3)\) in the AC graph constructed with prime moves.}
	\label{fig:ak_prime_persistence}
\end{figure}

==> app/reduction.tex <==
\section{Reduction}\label{app:families}

==> app/wirtinger.tex <==

The claimed trivialization of $AK(3)$ in \cite{shehper2024makesmathproblemshard} comes from demonstrating that $AK(3)$ is stably AC-equivalent to the following presentation from \cite{myasnikov2003andrewscurtisequivalence}:
\[
MMS3 := \langle x,y,z \,\, \mid \,\, x=z\cdot [[y^{-1},x^{-1}],z], y=x\cdot [[y^{-1},x^{-1}],z^{-1}]\cdot [z^{-1},x], x^{-1}yz\rangle.
\] 
The presentation $MMS3$ was believed to be stably AC-trivial because the first two relations were thought to be obtained from the Wirtinger presentation of the unknot in Figure~\ref{fig:unknot} from \cite{myasnikov2003andrewscurtisequivalence}. In \cite{myasnikov2003andrewscurtisequivalence}, the following purported presentation is given as the Wirtinger presentation of the unknot:
\[
\begin{aligned}
WWU=\left\langle x_1, x_2, x_3, x_4, x_5, x_6, x_7, x_8, x_9, x_{10}, x_{11}, x_{12}, x_{13}, x_{14} \right. \mid\, &x_1=x_{10} x_{14} x_{10}^{-1}, x_2=x_{10}^{-1} x_1 x_{10},\\
&x_3=x_1^{-1} x_2 x_1, x_4=x_6^{-1} x_3 x_6,\\
&x_5=x_{12} x_4 x_{12}^{-1},x_6=x_7^{-1} x_5 x_7, \\
&x_7=x_4^{-1} x_6 x_4, x_8= x_1 x_7 x_1^{-1}, \\
&x_9=x_{11}^{-1} x_8 x_{11}, x_{10}=x_{14} x_9 x_{14}^{-1} \\
&x_{11}=x_2^{-1} x_{10} x_2, x_{12}=x_1^{-1} x_{11} x_1 \\
& x_{13}=x_5 x_{12} x_5^{-1}, x_{14}=x_1 x_{13} x_1^{-1}\left. \right\rangle
\end{aligned}
\]

We obtain $MMS3$ after deleting the relation $x_{12}=x_1^{-1}x_{11}x_{1}$ and adding the relation $w=x^{-1}yz$, and then using substitution to simplify the presentation. 

Unfortunately, $WWU$ is not the Wirtinger presentation of the unknot in Figure~\ref{fig:unknot}. The error is that the relation $x_{13}=x_5 x_{12} x_5^{-1}$ is incorrect; it should instead be $x_{13}=x_4 x_{12} x_4^{-1}$. Indeed $WWU$ is not the Wirtinger presentation of any knot: in a Wirtinger presentation, any one relator is redundant, so a Wirtinger presentation with any relator removed is a presentation of the knot group—in the case an unknot, the infinite cyclic group $\mathbb{Z}$. Yet removing different relators from $WWU$ gives different groups. For example, if $x_7=x_4^{-1} x_6 x_4$ is eliminated, then the resulting group is the three-stand braid group, whereas if the relator $x_{14}=x_1 x_{13} x_1^{-1}$ is removed, we get $\mathbb{Z}$. Most importantly, however, the presentation $WWU$ with the relator $x_{12}=x_1^{-1}x_{11}x_1$ removed—the choice made in \cite{myasnikov2003andrewscurtisequivalence} that leads to $MMS3$—is not a presentation of $\mathbb{Z}$. 

Because of these facts, we cannot use Reidemeister moves to show the stable AC-triviality of $MMS3$ and therefore $AK(3)$ as well.  

The following fact may be of interest: 
Let $MMU(w)$ be $WWU$ with the relator $x_7=x_4^{-1} x_6 x_4$ eliminated, and with the added relator $w$ to trivialize the group. Then we have the following proposition: 

% We can drive a balanced presentation $MMSU$ of the trivial group from $WWU$.  
% The presentation $MMSU$ is an interesting balanced presentation of the trivial group: if it would be stably Andres-Curtis trivial, then we will show that the whole sequence of $AK(n)$ will be stably AC-trivial.

\begin{myprop}  The balanced presentation $MMU(w)$ of the trivial group is stably AC-equivalent to $\langle x,y \mid xyx=yxy, w\rangle$; in particular, for $w_n=x^{-n}y^{n+1}$, we have that $MMU(w_n)$ is stably AC-equivalent to
    $AK(n)$ for each $n\geq 1$. 
\end{myprop}


\begin{proof}

Eliminating the relator $x_7=x_4^{-1} x_6 x_4$, we add any word $w$ in $x_7$ and $x_{13}$ which trivializes the group. Note such a word will have exponent sum $\pm 1$. We show that this presentation is stably AC-equivalent to $\langle x,y \mid xyx=yxy, w\rangle$ for $x=x_7$ and $y=x_{13}$.

To do this, we first substitute $x_1=x_{10} x_{14} x_{10}^{-1}$ into the second relator to get $x_2=x_{14}$ and then eliminate $x_2$. Next from the third relator we have $x_{14}=x_{1} x_{3} x_1^{-1}$ and we substitute this into the relator $x_{14}=x_1 x_{13} x_1^{-1}$ to get $x_3=x_{13}$, and we eliminate $x_3$. Moreover, since the eleventh relator now reads $x_{11}=x_2^{-1} x_{10} x_2$ we substitute $x_{10}=x_{14}x_9x_{14}^{-1}$ to get $x_{11}=x_9$ and from this $x_9=x_8$ from the ninth relator.  Our presentation now reads
\[ \begin{aligned} \langle x_1, x_4, x_5, x_6, x_7, x_8, x_{10}, x_{12}, x_{13}, x_{14} \mid \, & x_1= x_{10} x_{14} x_{10}^{-1}, x_{13}= x_1^{-1} x_{14} x_{1}, x_4= x_6^{-1} x_{13} x_{6},\\
& x_5= x_{12} x_{4} x_{12}^{-1},x_6= x_7^{-1} x_{5} x_{7},x_8= x_{1} x_{7} x_1^{-1}, \\
&x_{10}= x_{14} x_{8} x_{14}^{-1}, x_{12}= x_1^{-1} x_{8} x_{1},x_{13}= x_{5} x_{12} x_5^{-1}, w\rangle  \end{aligned} \]

Now we substitute $x_8=x_1 x_7 x_1^{-1}$ into $x_{12}=x_1^{-1} x_8 x_1$ to get $x_{12}=x_7$ and we eliminate $x_{12}$. This now gives $x_5=x_7 x_4 x_7^{-1}$ which we substitute into $x_6= x_7^{-1} x_{5} x_{7}$ to get $x_6=x_4$ and from this we get $x_4=x_{13}$. We then eliminate $x_6$ and $x_4$. What remains is 

\[ \begin{aligned} \langle x_1, x_5, x_7, x_8, x_{13}, x_{14}\mid\, & x_1= x_{10} x_{14} x_{10}^{-1},x_{13}=x_1^{-1} x_{14} x_{1},x_8= x_{1} x_{7} x_1^{-1},\\
&x_{10}= x_{14} x_{8} x_{14}^{-1},x_5= x_{7} x_{13} x_7^{-1}, x_{13}= x_{5} x_{7} x_5^{-1}, w \rangle \end{aligned} \] 

Now we substitute $x_{10} = x_{14}x_8 x_{14}^{-1}$ into the first relator and eliminate $x_{10}$, followed by substituting $x_{14}=x_{1} x_{13} x_1^{-1}$ and eliminating $x_{14}$. We next substitute $x_8=x_1 x_7 x_1^{-1}$ and eliminate $x_8$, and then $x_5=x_7 x_{13} x_{7}^{-1}$ and eliminate $x_5$. We are left with 
\[ \langle x_1, x_7, x_{13} \mid  x_7 x_{13} x_7 = x_{13} x_7 x_{13}, x_1 = x_{13} x_7 x_{13} x_7^{-1} x_{13}^{-1}, w  \rangle \] which, after setting $x=x_7, y=x_{13}$ is stably AC-equivalent to 
\[
\langle x,y \mid xyx=yxy, w\rangle.
\]

Thus by setting $w=x^{-n}y^{n+1}$, we obtain the proposition.

\end{proof}




\begin{figure}
    \centering
\begin{tikzpicture}
\draw[thick] (0,0)--(1.8,0);
%x3
\draw[thick] (2.2,0)--(5.8,0);
%x2
\draw[thick,rounded corners] (6.2,0)--(7,0)--(7,1.5)--(2,1.5)--(2,-7)--(7,-7)--(7,-5)--(6.2,-5);
%x1
\draw[thick,rounded corners] (0,0)--(-2,0)--(-2,-0.8);
%x3
\draw[thick,rounded corners] (-2,-1.2)--(-2,-6)--(0,-6)--(0,-4.2);
%x4
\draw[thick,rounded corners] (0,-3.8)--(0,-2.2);
%x5
\draw[thick,rounded corners] (0,-1.8)--(0,-1)--(-3,-1)--(-3,-2)--(-2.2,-2);
%x6
\draw[thick,rounded corners] (-1.8,-2)--(1.8,-2);
%x7
\draw[thick,rounded corners] (1.8,-4)--(-1,-4)--(-1,-5)--(-0.2,-5);
%x12
\draw[thick,rounded corners] (0.2,-5)--(1.8,-5);
%x13
\draw[thick,rounded corners] (2.2,-4)--(4,-4)--(4,-0.2);
%x11
\draw[thick,rounded corners] (4,0.2)--(4,0.75)--(6,0.75)--(6,-6)--(5,-6)--(5,-5.2);
%x10
\draw[thick,rounded corners] (2.2,-5)--(5.8,-5);
%x14
\draw[thick,rounded corners] (5,-4.8)--(5,-2)--(4.2,-2);
%x9
\draw[thick,rounded corners] (2.2,-2)--(3.8,-2);
%x8

\node at (4.5,1.5){$>$};
\node at (3,0){$<$};
\node at (0,0){$<$};
\node at (-2,-3){\rotatebox{90}{$<$}};
\node at (0,-3){\rotatebox{90}{$>$}};
\node at (-1,-1){$<$};
\node at (1,-2){$>$};
\node at (3,-2){$>$};
\node at (4.5,-2){$>$};
\node at (6,-2.5){\rotatebox{90}{$>$}};
\node at (3,-4){$<$};
\node at (-0.5,-4){$<$};
\node at (1,-5){$>$};
\node at (3,-5){$>$};

\node at (4.5,2){$x_1$};
\node at (3,0.5){$x_2$};
\node at (0,0.5){$x_3$};
\node at (-2.5,-3){$x_4$};
\node at (0.5,-3){$x_5$};
\node at (-1,-0.5){$x_6$};
\node at (1,-1.5){$x_7$};
\node at (3,-1.5){$x_8$};
\node at (4.5,-1.5){$x_9$};
\node at (6.5,-2.5){$x_{10}$};
\node at (3,-3.5){$x_{11}$};
\node at (-0.5,-3.5){$x_{12}$};
\node at (1,-5.5){$x_{13}$};
\node at (3,-5.5){$x_{14}$};


\end{tikzpicture}
    \caption{Unknot diagram}
    \label{fig:unknot}
\end{figure}

==> sec/bartek_bfs.tex <==
% !TEX root = ../ac_paper.tex

\begin{algorithm}
	\caption{Breadth-First Search Algorithm}\label{alg:bfs}
	\begin{algorithmic}[1] % The number [1] ensures lines are numbered
		\State \textbf{Input:} A balanced presentation $\pi$, maximal size of presentation $n$
		\State \textbf{Output:} set of enumerated presentations connected to starting presentations that are achievable without exceeding size limit; and set of egdes with filtrations
		\State Initialize a queue $Q$, set of visited nodes $visited$, numerical map $name$ that will enumerate presentations
		\State Put $\pi$ as visited, into queue $Q$ and give it number $0$.
		\While{$Q$ is not empty}
		\State $u \gets $ top of $Q$
  \Comment{Remove the front node of $Q$}
		\For{every AC move $m$}
  \State $child \gets m(u)$
		\If{$child$'s size $\leq n$ and $child$ is not visited}
		\State put $child$ in $Q$ and into $visited$
  \State give $child$ next available number
		\EndIf
	\If{$child$ size $\leq n$ and $u$ number is smaller then the $child$'s number }
		\State return edge $(u, child)$ with proper filtration\EndIf
 
		\EndIf
		\EndFor
		\EndWhile
		
	\end{algorithmic}
\end{algorithm}


==> sec/future.tex <==
% !TEX root = ../ac_paper.tex

\section{Future Directions}

Our choice for maximum length that each relator is allowed to take could be enlarged. 

Include Theorem 1.4 of MMS and check if we can relate other examples of Akbulut-Kirby series to the presentations by picking different choices of w.

Use MCTS?

Change the initial state distribution in RL to include canonic presentations of certain lengths.

Scale RL?

Apply to other types of series such as Gordon's series?

Does stable AC equivalence imply AC equivalence? Explore this more.

There is also a length-14 presentation in \cite{MMS} for which the authors could not reduce the length of the relators using AC moves.
\[
\angles{x, y \mid xyx^{-2}y^{-1} xy^{-1}, x^{-1} y^{-1} x y^2 x y^{-1}}.
\]

There also exist other generalizations of the conjecture for other kinds of groups; some of which have been proved.
In particular, the conjecture holds true for finite groups and soluble groups \cite{Borovik, Guyot}.
I think these versions will not be important for us but can one learn algorithmic lessons from applying RL / GS to those cases?

 This paper says that either the Andrews Curtis conjecture is false or there is an algorithm to recognise balanced presentations of the trivial group: https://arxiv.org/pdf/math/0108053.pdf
Can we get more insight into Andrews-Curtis by using a Transformer classifier to distinguish balanced presentations much like knots and unknots have been distinguished before?

How do the number of solved presentations depend on the limit of maximum number of nodes given in the greedy search algorithm? 

How do the number of solved presentations depend on the maximum path length in proximal policy optimization?

Increase path length. Find a way to stably train that. 

It might be useful to try other architectures such as MCTS.

While we did some hyperparameter tuning, the analysis could be done in a much more systematic way. This would require a lot more compute but could be very useful. For example, it will be nice to estimate the critical batch size for optimization. It will also be nice to use the iteration batch-size invariance, i.e. PPO-EWMA so that we can perform our experiments at one iteration batch size. If we get more compute, we can scale the number of parallel actors (wait does iteration batch size tell us about number of parallel actors or horizon length or both?)

We need to strike a balance between the path length and the 

Scale?

==> sec/legacy.tex <==

\input{app/stable_ak3}

==> sec/n+11.tex <==
% !TEX root = ../ac_paper.tex

\subsection{Length reduction for $\AK(n)$}

Using the greedy search algorithm, we found a reduction of $\AK(5)$ to length $16$, using a little less than $20$ million nodes.
It was previously unknown whether any length reduction was possible for any of the presentations in the $\AK(n)$ sequence for $n \geq 3$.

By examining this reduction, we find that it can be generalized to show that $\AK(n)$, which has total relator length $2n+7$, is AC-equivalent to a presentation of length $n+11$. This is a reduction in length for every $n \geq 5$.
Explicitly, we will prove \autoref{t:n+11} stating that $\AK(n)$ is AC-equivalent to the presentation
\[
\langle x,y \mid y^{-1} x^2 y = x y^{-1} x \ , \ y x y = x y^{n-1} x \rangle.
\]

To do so we will prove the following two lemmas from which the theorem follows easily.

\begin{lemma}
    For any $k<n$, $\AK(n)$ is AC-equivalent to $MS(n, w_k)$ where $w_k = y^{-k} x^{-1} y x y$. 
    \todo{Is it clear that k must be less than n? Also can k be zero or negative? If k can be zero or negative, then does the induction argument below need a modification? Also, if k does not need to be bound by n, then we have obtained two infinite families of AC-trivial presentations, i.e. $MS(1, w_k)$ and $MS(2, w_k)$. I think that we don't need k < n bound. If we do, then we should remove the remark below.}
    \[
\MS(n, w_k) = \angles{x, y \mid x^{-1} y^n x = y^{n+1}, x = y^{-k} x^{-1} y x y}.
\]
\end{lemma}


\begin{proof}
    In \cite{MMS}, it is shown that $AK(n)$ is AC-equivalent to $MS(n, w_1)$. Thus, we show that for any $k<n-1$, $MS(n, w_k)$ is AC-equivalent to $MS(n, w_{k+1})$, and the result follows by induction.

    First, note that the first relation in $MS(n, w_k)$ can be rearranged in the following three ways:
    \begin{enumerate}[label=(\roman*)]
        \item $y^kxy^{-1}=y^{k-n}xy^n$
        \item $yxy^{-n}=y^{-(n-1)}xy$
        \item $y^{n-k}x^{-1}y^{-(n-1)}=y^{-(k+1)}x^{-1}y$
    \end{enumerate}

    Now, we can rearrange the relation $x=w_k$ to get $y^k x y^{-1}=x^{-1}yx$ and substitute from (i) to get $y^{k-n} x y^n = x^{-1}yx$. Then we rewrite this as $yxy^{-n}=xy^{k-n}x$ and substitute from (ii) to get $ y^{-(n-1)}xy= xy^{k-n}x$. Finally, we rewrite this as $y^{n-k}x^{-1}y^{-(n-1)}=xy^{-1}x^{-1}$ and substitute from (iii), which gives $y^{-(k+1)}x^{-1}y=xy^{-1}x^{-1}$ or equivalently $x=y^{-(k+1)}x^{-1}yxy=w_{k+1}$. 
\end{proof}

\begin{lemma}
    $MS(n, w_{n-1})$ is AC-equivalent to $\langle x,y \mid y^{-1} x^2 y = x y^{-1} x \ , \ y x y = x y^{n-1} x \rangle$.
\end{lemma}

\begin{proof}
    The relation $x=w_{n-1}$ in $MS(n, w_{n-1})$ can be equivalently expressed as
    \begin{enumerate}[label=(\roman*)]
        \item $y^{n-1}xy^{-1}=x^{-1}yx$
        \item $y^{-1}xy^{n-1}=xyx^{-1}$
    \end{enumerate}
    Writing the first relation of $MS(n, w_{n-1})$ as  $(y^{n-1}xy^{-1})y^{-1}=y^{-1}xy^{n-1}$, we substitute from (i) on the LHS and (ii) on the RHS. This gives $x^{-1}yxy^{-1}=xyx^{-1}$, which we can rearrange to get the result.
\end{proof}

\begin{remark}
As a corollary of Lemma 4, $MS(n, w_k)$ for each fixed $n$ is an infinite family of AC-equivalent presentations. As $\AK(1)$ and $\AK(2)$ are known to be AC-trivial, $MS(1, w_k)$ and $MS(2, w_k)$ are infinite families of AC-trivial presentations.
\end{remark}

\begin{remark}
In Lemma 5, we obtained a presentation that is AC equivalent to $MS(n, w_{n-1})$. It is possible to find various other length reductions of $AK(n)$ by applying the procedure in the proof of Lemma 5 to $MS(n, w_k)$ for $k < n-1$. 
\end{remark}



==> sec/related.tex <==
\subsection*{Related Work}

\textit{Reinforcement Learning for long-horizon, sparse-reward environments.} Long-horizon, sparse-rewards problems have been a persistent challenge in reinforcement learning (RL), as they require agents to explore efficiently and learn from delayed and infrequent feedback. Atari games such as Montezuma’s Revenge \cite{bellemare2013arcade}, which requires long-term planning to collect keys and open doors, and Pitfall! \cite{machado_ale} have exemplified these difficulties. 
Similarly, robotic tasks such as dexterous manipulation \cite{rajeswaran2017learning} require agents to learn complex sequences of actions with little intermediate feedback.

Several approaches have been developed to tackle long-horizon, sparse-reward problems, including intrinsic motivation \cite{pathak2017curiosity}, reward shaping \cite{ng_reward}, and hierarchical reinforcement learning (HRL) \cite{sutton_hrl_1999}. Intrinsic motivation techniques such as curiosity-driven exploration encourage agents to explore novel states even in the absence of external rewards. Reward shaping methods provide additional guidance to help bridge the sparse reward signal but require careful engineering to avoid unintended biases. HRL methods, including options frameworks \cite{sutton_hrl_1999}, hierarchical abstract machines \cite{parr_russell}, and feudal reinforcement learning \cite{dayan_hinton_frl, vezhnevets2017feudal} learn structured policies that decompose complex tasks into smaller sub-problems. More recently, memory-based approaches \cite{ecoffet2019go, badia2020uplearningdirectedexploration} have been employed to improve long-term planning in these challenging environments.

% \textit{}

\textit{Andrews--Curtis Conjecture}. Previous studies of the Andrews--Curtis conjecture have used various search algorithms, including genetic algorithms \cite{genetic}, breadth-first search \cite{bfs-ac}, and other more sophisticated algorithms \cite{Bowman-McCaul, Panteleev-Ushakov, krawiec2016distance}. 
%\cite{BurnsI} present a re-formulation of the conjecture in terms of an infinite set of moves called \textit{elementary M-transformations}.
 
% \textit{Measures of Hardness}. \shehper{@Anibal: are there any previous works related to measures of hardness that you know of? maybe base on toplogical data analysis. If not, we can remove this point.}


% \textbf{Research math problems as MDPs}

% \textbf{Long-horizon environments and reinforcement learning}

% \textbf{Search for unicorns}

% \textbf{Dynamic Action Spaces}

% \textbf{Relation of AC conjecture with Algebraic topology?}


% 


% \footnote{An brute-force search is impossible to execute as the size of the AC graph grows exponentially with the length of the sequence of AC moves. For a presentation with $n$ generators, the number of AC-moves is $3n^2$. The total number of sequences of AC-moves of length $l$ is $(3n^2)^l$. This number is already of the order $10^{21}$ in the modest case of $n=2$ and $l=20$.}

% Failure to solve a presentation using graph search should not be taken as strong evidence that the presentation is a genuine counterexample. There are known presentations where the trivializing sequence of AC moves grows as a superexponential function of the presentation's length \cite{Bridson, Lishak}. This highlights the need for innovative search and learning algorithms capable of addressing such long-horizon problems. Simultaneously, the Andrews--Curtis conjecture offers a useful testbed for evaluating the performance of these algorithms.

